From Soft Classifiers to Hard Decisions: How fair can we be?

A popular methodology for building binary decision-making classifiers in the presence of imperfect information is to first construct a non-binary "scoring" classifier that is calibrated over all protected groups, and then to post-process this score to obtain a binary decision. We study the feasibility of achieving various fairness properties by post-processing calibrated scores, and then show that deferring post-processors allow for more fairness conditions to hold on the final decision. Specifically, we show: 1. There does not exist a general way to post-process a calibrated classifier to equalize protected groups' positive or negative predictive value (PPV or NPV). For certain "nice" calibrated classifiers, either PPV or NPV can be equalized when the post-processor uses different thresholds across protected groups, though there exist distributions of calibrated scores for which the two measures cannot be both equalized. When the post-processing consists of a single global threshold across all groups, natural fairness properties, such as equalizing PPV in a nontrivial way, do not hold even for "nice" classifiers. 2. When the post-processing is allowed to `defer' on some decisions (that is, to avoid making a decision by handing off some examples to a separate process), then for the non-deferred decisions, the resulting classifier can be made to equalize PPV, NPV, false positive rate (FPR) and false negative rate (FNR) across the protected groups. This suggests a way to partially evade the impossibility results of Chouldechova and Kleinberg et al., which preclude equalizing all of these measures simultaneously. We also present different deferring strategies and show how they affect the fairness properties of the overall system. We evaluate our post-processing techniques using the COMPAS data set from 2016.

==> src/deferral_prelims.tex <==
% !TeX root = ../main.tex

\section{Deferral Preliminaries}
\label{sec:deferral_prelims}

In the first part of the paper, we considered the problem of post-processing calibrated soft classifiers, which output a score
$\score \in [0,1]$, into fair hard classifiers, which output a decision in $\py\in\{\pF,\pT\}$, subject to a number of group fairness conditions.
In the remainder of this work, we reconsider this problem, but with one important change: we allow classifiers to
``refuse to decide'' by outputting the special symbol $\punt$. We call such classifiers \emph{deferring} classifiers,
borrowing the nomenclature from \cite{MPZ17}. The output $\punt$ is the deferring classifier's way of refusing to make a decision and deferring to a downstream decision maker. For example, a risk assessment tool might aid a parole board to make a decision by categorizing an individual as high risk or low risk, or it might output $\punt$---providing no advice and deferring to the  judgment of the board.

We now modify our notation appropriately. Instances $x$ are still associated with a true type $\ty(x) \in \{\tF, \tT\}$ and a group $\group(x) \in \G$. A deferring hard classifier $\hard$ is a randomized function $\hard:\X \to \{\pF,\pT, \punt\}$.
A deferring soft classifier is a randomized function $\soft:\X\to[0,1]\cup \{\punt\}$.
A deferring hard (resp.~soft) post-processor is a randomized function $\post: [0,1]\cup\{\punt\} \times \G \to
\{\pF,\pT,\punt\}$ (resp.~$\postsoft: [0,1] \cup \{\punt\} \times \G \to [0,1] \cup \{\punt\}$) that takes as input the
output of a deferring soft and post-processes it into a deferring hard (resp.~soft) classifier.

\subsection{Types of downstream decision makers}
It's important to recognize that deferring does not fix unfairness, it only transforms it.
Ultimately, whether a deferring classifier is thought of as promoting fairness may depend on the nature of the downstream decision maker who must make decisions on instances which have been deferred.

One convenient yet often unrealistic scenario is a ``perfect'' downstream decision maker:
some procedure that is expensive to run but offers perfect (or near-perfect) accuracy.
A perfectly accurate downstream decision maker is ``fair'' in a number of ways: it offers perfect PPV, NPV, FPR, and FNR to all groups;furthermore, it is also individually fair--- treating likes alike.
The unfairness that remains in the overall system, therefore, is a function of the distribution of deferrals.

A somewhat more realistic scenario is a ``perfect-but-painful'' downstream decision maker.  This differs from the above in that it is costly not only to the entity making the decision, but also to the individual being decided upon. For example, an individual might receive accurate medical diagnoses only after being subjected to very invasive or harmful tests. The expense of deferral to the individual complicates our understanding of the fairness of the overall system.

Another likely scenario is that $\idk$ results are passed to a different, potentially
human decision-maker, which may not be as accurate as the original classifier (though is potentially inaccurate in an incomparable way). As in the earlier scenarios, unfairness may manifest itself in the decision to defer. However, there may be even greater unfairness to the deferred individuals. 

In either scenario, we may wish to minimize the total rate of deferrals, equalize it between groups, or restrict deferrals to a particular group.

\subsection{Statistical properties of deferring classifiers: contrasting approaches}

We wish to define statistical properties of deferring classifiers. While calibration, PPV, and NPV
apply to deferring classifiers without change, it is not clear how best to generalize the definitions of FPR and FNR, or more generally the error rate.

For example, recall the definition of the false positive rate (Definition~\ref{defn:four-measures}): The false positive rate of a (non-deferring) hard classifier $\hard$ for a group $g$ is $\FPR_{\hard,g} = \Pr[\hard(X_g) = \pT \mid \ty(X_g) = \tF]$.

One possible approach to incorporating deferrals is to condition on not deferring. That is, define the \emph{conditional false positive rate} as $\Pr[\hard(X_g) = \pT \mid \ty(X_g) = \tF, \hard(X_g) \neq \punt]$.
A deferring classifier $\hard$ that output $\pT$ on half of true negative instances (within a $g$) would have
conditional false positive rate as low as 0.5 (if it never output $\punt$ on true negatives) or as high as $1$ (if it
never output $\pF$ on true negatives). The conditional false positive rate is agnostic towards the downstream decision maker. It codifies no value judgments as to whether a deferral is desirable or undesirable as an individual nor whether deferrals ultimately result in accurate or inaccurate decisions.

A second approach is to leave the original definition unchanged. The same deferring hard classifier as above would have (ordinary, not conditional) false positive rate $\Pr[\hard(X_g) = \pT \mid \ty(X_g) = \tF] =0.5$. This would be true regardless of whether $\hard$ output $\pF$ or $\punt$ on the other half of true negative instances.
We call this the \emph{unconditional false positive rate}.
The unconditional false positive rate effectively categorizes deferrals as correct outputs. This may be appropriate if the downstream decision maker has very high accuracy. If, for example, a doctor orders an additional, more accurate diagnostic test in response to a deferral, the unconditional false positive rate might be appropriate.

Finally, a third approach is to base our measure of inaccuracy on the true negatives instead of the false positives.
Namely, we could consider $1-\Pr_{X \sam \X_g}[\hard(X) = \pF \mid \ty(X) = \tF]$. In contrast to the unconditional
false positive rate, this measure effectively categorizes deferrals as incorrect outputs. This may be appropriate if
the downstream decision maker has is inaccurate, or if a deferral is associated with significant cost to the
individual. Continuing the medical example, if the additional test requires an expensive and risky surgery, this third
approach might be most appropriate.

Just as in the case of non-deferring classifiers, the relationships among these contrasting group statistics, their meaningfulness in different settings, and their application in different settings are not well understood and deserve further study.

In this work, we focus on the conditional versions of false positive and negative rates.

\begin{definition}\label{defn:conditional-measures}
The \emph{conditional false positive rate}  and \emph{conditional false negative rate} of a deferring hard classifier $\hard$ for a group $g$ are, respectively: \[ \cFPR_{\hard,g} = \Pr[\hard(X_g) = \pT \mid \ty(X_g) = \tF, \hard(X_g) \neq \punt]. \]
\[ \cFNR_{\hard,g} = \Pr[\hard(X_g) = \pF \mid \ty(X_g) = \tT, \hard(X_g) \neq \punt]. \]
\end{definition}

We additionally consider a version of the distribution of calibrated scores conditioned on not deferring, which we call the \emph{conditional DOCS}. For non-deferring soft classifiers, Definitions~\ref{defn:conditional-docs} and \ref{defn:docs} coincide.
\begin{definition}
  \label{defn:conditional-docs}
 The \emph{conditional DOCS} $\pdf_g$ of a classifier $\soft$ for a group $g$ is the PMF of $\soft(X_g)$, conditioned on not outputting $\punt$. That is, for $\score \in [0,1]$,
 $\pdf_g(\score) =
 \Pr[\soft(X_g) = \score \mid \soft(X_g) \neq \punt].$ Note that the conditional DOCS is undefined if $\Pr[\soft(X_g) \neq \punt] = 0$.

 Abusing notation, we denote by $\pdf$ the collection $\{\pdf_g\}_{g\in \G}$, and call it the \emph{conditional DOCS of~\soft}.
\end{definition}

Because they make no assumptions about the behavior of the downstream decision maker, the conditional error rates are
applicable generally, but they can be difficult to interpret.
They are also amenable to the consideration of additional goals which we will briefly address. For example, one could seek
to minimize the total deferral rate, equalize the deferral rate among groups, or prefer deferrals on positive
instances.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

